Some theorems on decomposable continua

We prove some theorems on decomposable continua. In particular, we prove; (i) the property of being a Wilder continuum is not a Whitney reversible property, (ii) inverse limits of D**-continua with surjective monotone upper semi-continuous bonding functions are D**, and (iii) there exists a D**-continuum which contains neither Wilder continua nor D*-continua. Also, we show the existence of a Wilder continuum containing no D*-continua and a D*-continuum containing no Wilder continua.

==> d.tex <==
\begin{tikzpicture}[xscale=2,yscale=1.6]
\draw (1,0) ellipse (1.14 and 1.5);
\draw[domain=2.24:2.7,samples=100] plot (\x, {(1/(3))*\x*sin((8/(\x-2))r)});
\draw[domain=2.24:2.7,samples=100] plot (-\x+2, {(1/(3))*\x*sin((8/(\x-2))r)});
\draw (-.7,-0.8) to [out=270,in=180] (1,-2.5) to [out=0,in=270] (2.7,-0.8);
\draw[line width=1.75, domain=-26:26] plot ({1+1.14*cos(\x)},{1.5*sin(\x)});
\draw[line width=1.75, domain=154:206] plot ({1+1.14*cos(\x)},{1.5*sin(\x)});
\node at (1.9,0) {$\mathbf{}$};
\node at (0.1,0) {$\mathbf{}$};
\end{tikzpicture}
